Evidence for $X(3872)\rightarrow J/\psi \pi^+\pi^-$ produced in single-tag two-photon interactions

We report the first evidence for $X(3872)$ production in two-photon interactions by tagging either the electron or the position in the final state, exploring the highly virtual photon region. The search is performed in $e^+e^- \rightarrow e^+e^-J/\psi\pi^+\pi^-$, using 825 fb$^{-1}$ of data collected by the Belle detector operated at the KEKB $e^+e^-$ collider. We observe three $X(3872)$ candidates with an expected background of $0.11\pm 0.10$ events, with a significance of 3.2$\sigma$. We obtain an estimated value for $\tilde{\Gamma}_{\gamma\gamma}{\cal B}(X(3872)\rightarrow J/\psi\pi^+\pi^-$) assuming the $Q^2$ dependence predicted by a $c\bar{c}$ meson model, where $-Q^2$ is the invariant mass-squared of the virtual photon. No $X(3915)\rightarrow J/\psi\pi^+\pi^-$ candidates are found.

==> Makefile <==
FILE=Jpp

all :
	latex ${FILE}
	bibtex ${FILE}
	latex ${FILE}
	latex ${FILE}

bib :
	bibtex ${FILE}

plot :
	dvipdfmx -q -E -o ${FILE}.pdf ${FILE}.dvi
	qpdfview ${FILE}.pdf

file :
	dvipdfmx -q -E -o ${FILE}.pdf ${FILE}.dvi
	pdf2ps ${FILE}.pdf ${FILE}.ps

print :
	dvipdfmx -o ${FILE}.pdf ${FILE}.dvi
	pdf2ps ${FILE}.pdf ${FILE}.ps
	lpr -PHL-5450DN ${FILE}.ps

clean :
	rm -f ${FILE}.log ${FILE}.aux ${FILE}.dvi ${FILE}.bbl ${FILE}.blg \
	${FILE}Notes.bib

